White-box validation of quantitative product lines by statistical model checking and process mining

We propose a novel methodology for validating software product line (PL) models by integrating Statistical Model Checking (SMC) with Process Mining (PM). Our approach focuses on the feature-oriented language QFLan in the PL engineering domain, allowing modeling of PLs with rich cross-tree and quantitative constraints, as well as aspects of dynamic PLs like staged configurations. This richness leads to models with infinite state-space, requiring simulation-based analysis techniques like SMC. For instance, we illustrate with a running example involving infinite state space. SMC involves generating samples of system dynamics to estimate properties such as event probabilities or expected values. On the other hand, PM uses data-driven techniques on execution logs to identify and reason about the underlying execution process. In this paper, we propose, for the first time, applying PM techniques to SMC simulations' byproducts to enhance the utility of SMC analyses. Typically, when SMC results are unexpected, modelers must determine whether they stem from actual system characteristics or model bugs in a black-box manner. We improve on this by using PM to provide a white-box perspective on the observed system dynamics. Samples from SMC are fed into PM tools, producing a compact graphical representation of observed dynamics. The mined PM model is then transformed into a QFLan model, accessible to PL engineers. Using two well-known PL models, we demonstrate the effectiveness and scalability of our methodology in pinpointing issues and suggesting fixes. Additionally, we show its generality by applying it to the security domain.

==> introBackup.tex <==
\section{Introduction}
\label{sec:intro}
%State the objectives of the work and provide an adequate background, avoiding a detailed literature survey or a summary of the results.

% \comal{After a discussion with Andrea B. and having read the entire paper, I would suggest to include the example of Fig.~\ref{fig:abstract_example} or a similar one and tell the story using it.} \comr{Ho aggiunto l'esempio astratto in questa sezione}

Software product lines (SPL), and feature models in general, as well as Product Line Engineering (PLE), play a very important role in modern society, where customization capabilities are expected even for commodity products. Very often, these products are equipped with software that is expected to follow the customization of the product itself. As a consequence, it becomes necessary to ensure that the product lines are properly designed and that the models indeed capture the intentions of the modelers. This paper presents a novel methodology to validate the behavior of SPL models by offering simple tools to ``see and compare'' the \emph{actual} behavior of a model with the \emph{expected} one.

To validate models that present quantitative aspects in their behavior, we often use numerical and statistical analysis techniques. 
The formal verification of the dynamics of a system via numerical techniques provides precise values of the (quantitative) properties being analyzed. These typically require reasoning upon the whole behavior of the system, which might not be feasible for complex models. Indeed, as the possible dynamics of the system increase, these techniques tend to suffer from the well-known state-space explosion problem. %become increasingly computationally demanding, making them more appropriate for smaller systems. 
On the other hand, statistical analysis techniques, such as Statistical Model Checking (SMC)~\cite{Agha18}, rely only on limited but statistically relevant samples of executions of a model: simulations. Therefore, statistical analysis techniques can be used to analyze complex dynamical systems at the cost that analysis results are not \emph{exact} anymore but are statistically reliable estimations, e.g., equipped with confidence intervals.

When the overarching behavior of a system is unknown, and it is impossible to make assumptions about its transition structure, the system is referred to as a black-box system. An SMC that analyzes the dynamics of a black-box system without prior knowledge of the system is referred to as a black-box SMC~\cite{younes2005probabilistic}. These simulation-based approaches return numerical estimates, plots, and occasionally counterexamples of the studied properties. However, they typically do not provide behavioral explanations for the results obtained. Without clear explanations, the modeler can only make informed guesses about how to adjust the model to fix unwanted behaviors. For example, let us assume that we consider an SPL model for a family of coffee machines, a classic PLE model (see, e.g.,~\cite{BMS12,CHSLR10}). Let us further assume that we use black-box SMC to study the probability that machines from the family contain dispensers for cappuccino, and that we get $0$. Interesting questions are: 
\begin{itemize}
	\item \emph{What is the reason behind such an extreme value?}, 
	\item \emph{Was the model intended to express this dynamics, or is there a bug?}
\end{itemize}
%\comal{It would be nice to mention a concrete example here.}
%\comb{Agreed, but I don't have one now, tho. Roberto? Andrea?}\coma{It shall be one of those used in validation. Coffee machine is good, I think. But I was not able to write it in less text...}

Process Mining (PM) is a process-oriented data-driven technique that analyzes the executions (i.e., traces) of activities generated by information systems, allowing the identification of process patterns, bottlenecks, and other issues in a model~\cite{VanderAalst2016}. Visualizing the flow of activities helps identify opportunities for improvement (e.g., unexpected loops or unexpected dependencies).

%\comal{Lo sposto alla fine} \comal{Non ricordo avere scritto questo commento. Per me si puo' ignorare.}\coma{l'avevo scritto io :D lasciamo qui, ok}
This paper, which extends a preliminary work~\cite{10.1007/978-3-031-25383-6_18} where we demonstrated the potential of enriching SMC techniques with Process Mining, presents a white-box technique to enable the evaluation of behavioral aspects of a feature model. The technique leverages the application of process mining techniques on event logs produced by (simulations generated by) statistical model checking. The goal is to provide insights into the system behavior, such as discovering new patterns, identifying bottlenecks, and improving the general model accuracy.  Therefore, integrating SMC with PM paves the way to a more comprehensive understanding of the overall behavior of the model and can help identify issues or suggest actionable improvements to the modeler. To the best of our knowledge, our methodology is the first attempt in \rev{automatically} \emph{explaining} the results of SMC using PM-based approaches. % \rev{applied on SPL models}. 
%
In our previous work, we showed the capabilities of analyzing traces generated by SMC with PM. However, the identification of issues was entirely delegated to the modeler's visual skills and hence highly subjective.  In the presence of a large model, mining the simulations would result in a complex model, making it difficult for the modeler to locate issues. 
Furthermore, we did not tailor the SPL domain, but only the cybersecurity one, while we now explicitly target the SPL domain by applying the approach on the feature-oriented language QFLan~\cite{DBLP:journals/tse/BeekLLV20,DBLP:conf/fm/VandinBLL18}.
In this paper, we overcome this limitation by \emph{automatically} discovering undesirable behaviors in the model specification itself. This is accomplished by highlighting the differences between the expected behavior of the model, the model specification, and the actual behavior discovered by mining its simulations. In fact, by highlighting the specific behaviors causing issues in the model, the modeler can make more targeted and effective adjustments to the model to fix those issues. %Furthermore, we now explicitly target the SPL domain by applying the approach on the feature-oriented language QFLan~\cite{DBLP:journals/tse/BeekLLV20,DBLP:conf/fm/VandinBLL18}.



\begin{figure}
	\centering
	\includegraphics[width=\textwidth]{images/abstract-example.pdf}
	\caption{Example of the input and output produced by the technique presented in this paper. The input model is simulated with SMC techniques and corresponding traces are used to synthesize a new model which is then compared to the original one and an easy-to-read output is returned to the modeller emphasizing the differences.}
	\label{fig:abstract_example}
\end{figure}
Figure~\ref{fig:abstract_example} illustrates an abstract example of a model validated using our method. The input model is a representation of an abstract  model. % produced by the modeling tool during the model creation phase. 
This abstract model includes different states and actions used to move between those states. In this example, the simulator would start from the node \cf{A} and with the \cf{ActionB} move to the node \cf{B}, and from there can move to another node by choosing the corresponding action. Without our methodology, %the modeler does not have much support for validation: they 
an SMC user would need to validate the input model using only the obtained numerical results (e.g., if interested in ``estimating the probability of reaching a specific node in the model''). With our approach, however, the modeler can inspect the results of the simulation once they are synthesized into new models, thus using the same language (i.e., models-to-model rather than models-to-numbers). The first graph in the ``output models'' box of Figure~\ref{fig:abstract_example} depicts the reconstructed model after applying Process Mining to the simulations. Instead,  the rightmost model depicts the graph obtained by comparing the input model and the reconstructed one. This final representation, in particular, highlights the differences between the input model and the simulated behavior, allowing the modeler to quickly identify issues, such as unexpected or missing behaviors. The exact semantics of the different colors of the edges is explained in Section~\ref{sec: method}.
It is worth mentioning that this method can, in principle, be applied to any discipline where discrete-state simulation models are used, enhancing the capabilities of related  modeling and analysis tools. On the other hand, the methodology is particularly useful for domains where the complexity of models is high, as in the case of highly-parametric models from PLE.
%\comal{questo è positivo, ma allo stesso tempo questa è una special issue su SPL. Il paper è partito con un paragrafo SPL e dopo 4 pagine il paper non dice ancora nulla di specifico su SPL. Quindi aggiungerei una frase tipo ``On the other hand, the methodology is particularly useful for domains where the complexity of models is high, as in the case of highly-parametric models from Product Line Engineering (PLE). ''. Se si aggiunge usare l'acronimo sotto (senza espanderlo).}


It is important to stress that the methodology depends on the input  model, but also on the chosen studied property, as this will drive the simulation process. This is somehow reminiscent of the so-called \emph{CEGAR} (counterexample guided abstraction and refinement~\cite{10.1007/10722167_15}) approaches from qualitative model checking \rev{(and also applied to probabilistic settings~\cite{DBLP:conf/cav/HermannsWZ08})}. In classic qualitative model checking, if the studied property does not hold, we get counterexamples of systems' dynamics that showcase executions that falsify the formula. CEGAR involves the use of such counterexamples to refine the model. In our methodology, we proceed similarly, by using mined process models as counterexamples.


% \begin{figure*}
	%     \centering
	%     \includegraphics[width=\textwidth]{images/abstract-example.pdf}
	%     % \begin{subfigure}[b]{0.28\textwidth}
		%     %     \centering
		%     %     \includegraphics[height=1\textwidth]{images/abstract_example_original.pdf}
		%     %     \caption{}
		%     %     \label{fig:original_behavior}
		%     % \end{subfigure}
	%     % \hfill
	%     % \begin{subfigure}[b]{0.28\textwidth}
		%     %     \centering
		%     %     \includegraphics[height=1\textwidth]{images/abstract_example_simulated.pdf}
		%     %     \caption{}
		%     %     \label{fig:simulated_behavior}
		%     % \end{subfigure}
	%     % \hfill
	%     % \begin{subfigure}[b]{0.28\textwidth}
		%     %     \centering
		%     %     \includegraphics[height=1\textwidth]{images/abstract_example_diff.pdf}
		%     %     \caption{}
		%     %     \label{fig:diff_behavior}
		%     % \end{subfigure}
	%     % \caption{Original model's behavior (a)
		%     %         Simulated model's behavior (b)
		%     %         Diff model's behavior (c)} %\comal{it would be fantastic to use something like this in the introduction. You can really tell the story of the paper with it and motivate the reader to read this long paper of how to achieve the nice highlight of the diff automatically}}
%     %         \label{fig:abstract_example}
%     \caption{Example of the input and output produced by the technique presented in this paper. The input model is simulated with SMC techniques and corresponding traces are used to synthesize a new model which is then compared to the original one and an easy-to-read output is returned to the modeller emphasizing the differences.}
%     \label{fig:abstract_example}
% \end{figure*}
% Our method offers a valuable solution for improving the formal verification of simulation models. It allows for a more comprehensive understanding of the model's overall behavior, enables the automatic discovery of undesirable behaviors, and facilitates the identification and fixing of issues in the model. Furthermore, this method can be widely applied to various disciplines where simulation models are used and can enhance the capabilities of existing modeling and analysis tools.

To validate our methodology we provide positive answers to the following research questions:
\begin{itemize}
\item[RQ1.] \textit{(effectiveness)} Can the developed techniques be used to identify errors in the simulation models? To answer this question, we apply our methodology to the feature-oriented quantitative modeling and analysis framework QFLan~\cite{DBLP:journals/tse/BeekLLV20,DBLP:conf/fm/VandinBLL18}. 
%framework belonging to the same family of feature-oriented specification languages, namely QFLan and RisQFLan~\cite{DBLP:conf/fm/VandinBLL18, ter2021quantitative}. 
We demonstrate the effectiveness of the proposed method by applying it to a model describing a family of beverage vending machines product line from~\cite{DBLP:conf/fm/VandinBLL18}, a classic case study in PLE. %\comal{mention that this is the classical case study in PLE?}
Our experiments %on the formal model describing the production line of a classic Coffee and Tea -based vending machine 
demonstrate the effectiveness of our method: We can automatically  detect which parts of the model behavior are missing.
%
\item[RQ2.] \textit{(scalability)} Are the developed techniques scalable to large models considered challenging by the SPL community? To answer this question we apply our methodology to a case study of an Elevator product line from~\cite{DBLP:journals/tse/BeekLLV20}, initially proposed by~\cite{PLATH200153}, which is a well-known case study used to test the scalability in PLE. %\comal{mention that this is one of the examples used to test scalability in PLE?}
Our experiments show that our methodology tends to have a runtime in the same order of magnitude of SMC analysis, and it never exceeds more than 5 times its runtime.
%
\item[RQ3.] \textit{(multi-domain)} Can the developed techniques generalize to further domains beyond software product lines? To answer this question we consider an additional domain, namely cybersecurity, using the framework RisQFLan~\cite{ter2021quantitative}. It is an incarnation  of QFLan to the cybersecurity domain. %
Thanks to this, we successfully validate our approach on an example of a threat model from~\cite{ter2021quantitative}, demonstrating its applicability to different domains.
%
Indeed, our we show how we automatically discovered unwanted and unexpected behaviors. In addition, we also got hints on how to fix such issues obtaining a refined model that does not show the issues.
\end{itemize}

\rev{All models and replication material for this paper are available at \url{https://doi.org/10.5281/zenodo.8225148}.}

The remainder of the paper is structured as follows. Section~\ref{sec:back} introduces necessary background material, as well as the coffee machine a running example. After this, Section~\ref{sec: method} presents our methodology, while Sections~\ref{subsec: effectiveness}-~\ref{subsec: Multi-domain} validates it on three case studies, answering our research questions. \rev{Section~\ref{sec:related} discusses related works, while} Section~\ref{sec:disc} concludes the paper 
and drafts future works. %\comb{Let's not forget this, but let's keep it as last part, once structure is finalized}
%First, Section ...

%\coma{Explain how we extended it here: we added QFLan to RisQFLan, we completed the methodology 'closing the loop'. We validated the methodology on the three dimensions presented in the next section via new experiments (we didn't validate it in DEC2H).}

% \section{Related work and research questions }
% \label{sec: research questions}

%\comal{I am not used to see related work and research questions together. I would expect research questions to be part of the introduction, right after the problem statement.}

% Some related work on product lines and data-driven approaches for them.\ldots

% Somehow connect the related work with the research questions

% \begin{itemize}
% \item[RQ1.] Can the developed techniques be used to identify errors in the simulation models? [effectiveness] 
% \item[RQ2.] Are the developed techniques scalable to larger models? [scalability] 
% \item[RQ3.] Can the developed techniques be used in different domains? [multi-domain] 
% \end{itemize}

%\comal{C'è una lettura ``empirical software engineering'' di RQ1 e RQ3 (quanto in pratica il tool sviluppato sia migliore che l'ispezione puramente visuale del previous work) che immagino non vada affrontata in questo paper. Forse è implicitamente banele? Vale la pena dirlo?}

%\comb{Spostare paragrafo su estensione paper qui? Also, aggiungere frase che "to best of our knowledge this is the only paper that"}
